Unsupervised anomaly detection algorithms on real-world data: how many do we need?

In this study we evaluate 32 unsupervised anomaly detection algorithms on 52 real-world multivariate tabular datasets, performing the largest comparison of unsupervised anomaly detection algorithms to date. On this collection of datasets, the $k$-thNN (distance to the $k$-nearest neighbor) algorithm significantly outperforms the most other algorithms. Visualizing and then clustering the relative performance of the considered algorithms on all datasets, we identify two clear clusters: one with ``local'' datasets, and another with ``global'' datasets. ``Local'' anomalies occupy a region with low density when compared to nearby samples, while ``global'' occupy an overall low density region in the feature space. On the local datasets the $k$NN ($k$-nearest neighbor) algorithm comes out on top. On the global datasets, the EIF (extended isolation forest) algorithm performs the best. Also taking into consideration the algorithms' computational complexity, a toolbox with these three unsupervised anomaly detection algorithms suffices for finding anomalies in this representative collection of multivariate datasets. By providing access to code and datasets, our study can be easily reproduced and extended with more algorithms and/or datasets.

==> Tables/AUC_global_datasets.tex <==
\begin{tabular}{llllllllllllllllllllllllll}
\toprule
{} & annthyroid & arrhythmia &    cardio &     cover & hepatitis &      http & internetads & mammography &     mnist &      musk & optdigits & pageblocks & pen-global & pendigits &      pima & satellite & satimage-2 & seismic-bumps &   shuttle &      smtp &  spambase &    stamps &   thyroid &       wbc &      wine \\
\midrule
ABOD    &    0.89604 &   0.812372 &  0.733892 &  0.791068 &  0.769231 &  0.967065 &    0.748419 &    0.785279 &   0.80132 &  0.164538 &  0.483381 &   0.940789 &   0.965351 &  0.754606 &  0.703351 &  0.969558 &   0.924613 &       0.73825 &  0.919925 &  0.953884 &  0.513733 &  0.843407 &   0.98233 &  0.963585 &  0.695798 \\
IF      &   0.650356 &   0.806014 &  0.928448 &   0.88407 &  0.695752 &  0.990474 &    0.689786 &    0.820926 &  0.806695 &       1.0 &  0.739371 &   0.899804 &   0.929712 &  0.953256 &  0.672112 &  0.952198 &   0.994579 &      0.672645 &  0.997869 &  0.927217 &  0.619945 &  0.894874 &  0.976382 &  0.981637 &  0.819328 \\
COPOD   &   0.701982 &   0.799772 &   0.92551 &  0.884081 &  0.803674 &  0.994552 &    0.676404 &    0.868517 &  0.773868 &   0.94634 &  0.680842 &   0.875374 &   0.785175 &  0.904805 &  0.654015 &  0.894008 &   0.974435 &      0.712603 &  0.996046 &  0.925294 &  0.677218 &   0.93016 &  0.937382 &  0.990974 &  0.867227 \\
ODIN    &   0.501237 &   0.638895 &  0.578355 &   0.52077 &  0.695178 &   0.49902 &    0.583084 &    0.620239 &  0.625537 &  0.562628 &  0.512584 &   0.592689 &   0.693833 &  0.512789 &  0.567948 &  0.493318 &   0.553369 &      0.539219 &  0.492868 &  0.440132 &  0.526301 &  0.605491 &  0.579577 &  0.812815 &  0.758403 \\
COF     &    0.36746 &   0.669728 &  0.521329 &  0.506718 &  0.629162 &  0.605982 &    0.679035 &    0.644876 &  0.610286 &  0.466463 &  0.494762 &   0.595726 &    0.67606 &  0.520788 &  0.612896 &  0.677058 &   0.569506 &      0.546961 &  0.593963 &  0.495571 &  0.466072 &  0.500261 &  0.495773 &  0.954248 &  0.421008 \\
kNN     &   0.904998 &   0.805582 &  0.827975 &  0.793385 &  0.794489 &  0.998432 &    0.738958 &    0.791247 &   0.81585 &  0.573895 &  0.479772 &   0.946984 &   0.988409 &  0.801176 &  0.714425 &  0.974417 &   0.963892 &      0.733855 &   0.95245 &   0.96078 &  0.661586 &  0.874935 &  0.986329 &  0.975412 &  0.891597 \\
HBOS    &   0.576633 &   0.800165 &  0.800836 &  0.636475 &  0.777268 &   0.97938 &    0.680901 &    0.796687 &  0.347673 &       1.0 &   0.87021 &   0.753965 &   0.774311 &  0.928866 &   0.69828 &  0.924889 &   0.975614 &      0.711484 &  0.953465 &  0.825633 &  0.643693 &  0.912935 &  0.967998 &  0.976657 &  0.907563 \\
LODA    &    0.68011 &   0.674812 &  0.867437 &   0.93795 &  0.633754 &  0.977835 &    0.649335 &    0.845405 &  0.412014 &  0.986141 &  0.676279 &   0.724188 &   0.681337 &   0.93095 &  0.632205 &  0.894291 &   0.985219 &      0.668489 &  0.952924 &  0.830586 &  0.428425 &  0.876605 &    0.7895 &  0.770931 &  0.771429 \\
MCD     &    0.91781 &   0.763738 &  0.822722 &  0.863835 &  0.786452 &  0.999731 &    0.799687 &    0.754617 &  0.860421 &  0.999694 &  0.419943 &   0.926786 &   0.911188 &  0.863628 &  0.680522 &  0.948979 &   0.992908 &      0.736838 &  0.991092 &  0.960816 &  0.482998 &  0.875666 &  0.987862 &  0.959851 &  0.960504 \\
LOF     &   0.414229 &   0.633812 &   0.54513 &  0.502542 &  0.707233 &  0.753614 &    0.658933 &    0.687327 &  0.618948 &  0.652176 &  0.516988 &   0.687147 &   0.760446 &  0.538625 &  0.606731 &  0.780247 &   0.621917 &      0.535152 &  0.671059 &  0.765995 &  0.504007 &  0.630024 &   0.63593 &  0.980703 &  0.878992 \\
OCSVM   &   0.948467 &   0.798516 &  0.875236 &  0.930268 &  0.765786 &  0.999861 &    0.689049 &    0.815663 &  0.764523 &  0.881271 &  0.518008 &   0.929568 &   0.874404 &  0.935421 &  0.640097 &  0.912352 &   0.988835 &      0.711792 &  0.987374 &  0.966734 &  0.523293 &  0.888506 &  0.985728 &  0.976346 &  0.878151 \\
LMDD    &   0.838772 &   0.816337 &  0.762342 &  0.834852 &  0.745121 &  0.999552 &    0.665142 &     0.78157 &  0.751749 &  0.970063 &  0.583077 &   0.774861 &   0.756267 &  0.929654 &  0.693769 &  0.681355 &    0.52965 &      0.664342 &  0.993534 &  0.951321 &  0.510323 &  0.904374 &  0.987953 &    0.9723 &  0.862185 \\
PCA     &   0.571938 &   0.774965 &  0.949623 &  0.935623 &  0.771527 &  0.999592 &    0.614632 &    0.743056 &  0.848756 &  0.999899 &  0.464645 &    0.89509 &   0.763185 &  0.924814 &  0.577761 &  0.846035 &   0.972936 &      0.649128 &  0.993458 &  0.945464 &  0.553171 &  0.887045 &  0.953144 &   0.97728 &  0.722689 \\
ECOD    &   0.775684 &   0.822657 &  0.952759 &  0.932698 &  0.786452 &   0.99379 &    0.676702 &    0.784675 &  0.838077 &  0.955011 &  0.615084 &   0.907428 &     0.7855 &  0.920638 &  0.517313 &  0.749199 &   0.973561 &      0.672161 &  0.996885 &  0.907017 &  0.644759 &  0.927341 &  0.975579 &  0.914706 &  0.710084 \\
SOD     &   0.796193 &   0.770765 &  0.709678 &  0.630655 &  0.548794 &  0.773319 &    0.568714 &    0.750524 &  0.698847 &  0.467548 &  0.560895 &   0.802164 &   0.903621 &   0.67793 &  0.572791 &  0.897141 &   0.831212 &      0.700512 &   0.80525 &  0.924862 &  0.586683 &   0.81021 &  0.957892 &  0.943978 &  0.596639 \\
u-CBLOF &   0.863022 &   0.791333 &  0.769888 &   0.89637 &  0.493111 &  0.999962 &    0.688946 &    0.726101 &  0.825099 &  0.966277 &  0.604703 &   0.935068 &   0.954998 &  0.948382 &  0.660612 &   0.96067 &   0.998736 &       0.69464 &  0.993248 &  0.955207 &   0.61137 &  0.716881 &  0.990337 &  0.956427 &  0.460504 \\
CBLOF   &     0.1416 &   0.413173 &  0.186039 &  0.815297 &  0.261768 &  0.096379 &    0.384746 &    0.350738 &  0.650494 &  0.092015 &  0.610337 &   0.355515 &    0.30178 &  0.485163 &  0.410739 &  0.483899 &   0.486015 &      0.300235 &  0.149748 &  0.068696 &  0.522523 &  0.254933 &  0.439982 &  0.129474 &  0.063866 \\
EIF     &   0.867758 &   0.818967 &  0.932896 &  0.892547 &  0.730195 &  0.992133 &    0.677355 &    0.818895 &   0.81332 &       1.0 &  0.659532 &    0.90152 &   0.934556 &   0.95128 &  0.688664 &  0.706723 &   0.995866 &      0.695571 &  0.997953 &  0.944912 &  0.653115 &  0.890176 &  0.982674 &  0.953221 &  0.846218 \\
\bottomrule
\end{tabular}


==> Tables/AUC_local_datasets.tex <==
\begin{tabular}{llllllllll}
\toprule
{} & parkinson &      wilt &      aloi &    vowels &    letter & pen-local &  waveform &     glass & ionosphere \\
\midrule
ABOD    &  0.640873 &  0.694148 &  0.617839 &  0.971751 &  0.832565 &  0.961776 &  0.696205 &  0.816449 &   0.932373 \\
IF      &  0.502268 &  0.441378 &  0.539757 &  0.782006 &  0.631369 &  0.776106 &  0.724055 &  0.703704 &   0.858311 \\
COPOD   &  0.535006 &  0.344711 &  0.515223 &  0.510066 &  0.559118 &  0.524892 &  0.733249 &  0.645969 &   0.802133 \\
ODIN    &   0.43006 &  0.673064 &   0.72942 &  0.884169 &   0.85509 &  0.879771 &  0.666017 &  0.720588 &   0.866222 \\
COF     &  0.623583 &  0.639706 &  0.766989 &  0.962567 &  0.863888 &  0.968658 &  0.723191 &  0.846405 &    0.87776 \\
kNN     &  0.629252 &  0.691692 &  0.589491 &  0.968365 &  0.845825 &  0.983286 &  0.745396 &  0.826253 &   0.919076 \\
HBOS    &  0.524943 &  0.362389 &  0.499594 &  0.668347 &  0.595631 &  0.733547 &  0.684587 &  0.675381 &   0.759289 \\
LODA    &  0.747662 &  0.407548 &  0.525897 &  0.772775 &  0.517422 &  0.554268 &  0.534882 &  0.240196 &   0.515556 \\
MCD     &  0.620607 &  0.860109 &  0.534613 &  0.919816 &  0.819586 &  0.760763 &  0.592334 &  0.739651 &   0.949156 \\
LOF     &  0.543509 &  0.650569 &  0.746232 &   0.94358 &  0.868243 &  0.988142 &  0.731717 &  0.825163 &   0.898987 \\
OCSVM   &  0.447279 &  0.445188 &  0.532609 &  0.723267 &  0.604616 &  0.485878 &  0.662273 &   0.69281 &   0.842524 \\
LMDD    &  0.616071 &  0.401765 &  0.498372 &  0.615468 &  0.527508 &  0.427037 &  0.606907 &  0.533769 &   0.712373 \\
PCA     &  0.264314 &  0.293839 &  0.551173 &  0.602928 &  0.517422 &   0.19206 &  0.503238 &  0.462418 &   0.807751 \\
ECOD    &  0.410998 &   0.42162 &    0.5349 &  0.410693 &  0.532884 &  0.445881 &  0.719199 &  0.683551 &   0.769493 \\
SOD     &  0.748299 &  0.596829 &  0.652294 &  0.942931 &  0.884242 &  0.967853 &  0.646658 &  0.795207 &   0.910649 \\
u-CBLOF &  0.610261 &  0.581602 &  0.530954 &  0.901061 &  0.801142 &  0.908849 &  0.694879 &  0.843682 &   0.920924 \\
CBLOF   &  0.564484 &  0.688412 &  0.537257 &    0.6604 &  0.661102 &  0.935856 &  0.590439 &  0.462418 &   0.641564 \\
EIF     &  0.514881 &  0.473199 &  0.535901 &  0.798751 &  0.628051 &  0.788276 &  0.743305 &  0.699346 &   0.875449 \\
\bottomrule
\end{tabular}


==> Tables/nemenyi_summary.tex <==
\begin{tabular}{lllllllllllllllllllllllllllllllll}
\toprule
{} & CBLOF & sb-DeepSVDD & SO-GAAL & ALAD & COF & DeepSVDD & ODIN & LOF & ensemble-LOF &   GMM &  LMDD &  LODA &   SOD &   PCA &  ECOD &   VAE & beta-VAE & LUNAR &    AE & OCSVM &  HBOS & COPOD & u-CBLOF &  ABOD & gen2out &   KDE &  INNE &   MCD &    IF &   kNN & kth-NN &   EIF \\
\midrule
EIF          &    ++ &          ++ &      ++ &   ++ &  ++ &       ++ &   ++ &  ++ &           ++ &       &    ++ &    ++ &    ++ &    ++ &       &       &          &       &       &       &       &       &         &       &         &       &       &       &       &       &        &       \\
kth-NN       &    ++ &          ++ &      ++ &   ++ &  ++ &       ++ &   ++ &  ++ &           ++ &       &    ++ &    ++ &    ++ &    ++ &       &     + &       ++ &       &       &       &       &       &         &       &         &       &       &       &       &       &        &       \\
kNN          &    ++ &          ++ &      ++ &   ++ &  ++ &       ++ &   ++ &  ++ &           ++ &       &    ++ &    ++ &    ++ &    ++ &       &       &          &       &       &       &       &       &         &       &         &       &       &       &       &       &        &       \\
IF           &    ++ &          ++ &      ++ &   ++ &  ++ &       ++ &   ++ &  ++ &           ++ &       &       &     + &       &    ++ &       &       &          &       &       &       &       &       &         &       &         &       &       &       &       &       &        &       \\
MCD          &    ++ &          ++ &      ++ &   ++ &  ++ &       ++ &   ++ &  ++ &              &       &       &       &       &       &       &       &          &       &       &       &       &       &         &       &         &       &       &       &       &       &        &       \\
INNE         &    ++ &          ++ &      ++ &   ++ &  ++ &       ++ &   ++ &  ++ &              &       &       &       &       &       &       &       &          &       &       &       &       &       &         &       &         &       &       &       &       &       &        &       \\
KDE          &    ++ &          ++ &      ++ &   ++ &  ++ &       ++ &   ++ &  ++ &           ++ &       &     + &    ++ &     + &    ++ &       &       &          &       &       &       &       &       &         &       &         &       &       &       &       &       &        &       \\
gen2out      &    ++ &          ++ &      ++ &   ++ &  ++ &       ++ &   ++ &  ++ &              &       &       &       &       &       &       &       &          &       &       &       &       &       &         &       &         &       &       &       &       &       &        &       \\
ABOD         &    ++ &          ++ &      ++ &   ++ &  ++ &       ++ &   ++ &  ++ &            + &       &       &       &       &       &       &       &          &       &       &       &       &       &         &       &         &       &       &       &       &       &        &       \\
u-CBLOF      &    ++ &          ++ &      ++ &   ++ &  ++ &       ++ &   ++ &     &              &       &       &       &       &       &       &       &          &       &       &       &       &       &         &       &         &       &       &       &       &       &        &       \\
COPOD        &    ++ &          ++ &      ++ &   ++ &  ++ &       ++ &   ++ &  ++ &              &       &       &       &       &       &       &       &          &       &       &       &       &       &         &       &         &       &       &       &       &       &        &       \\
HBOS         &    ++ &          ++ &      ++ &   ++ &  ++ &       ++ &   ++ &     &              &       &       &       &       &       &       &       &          &       &       &       &       &       &         &       &         &       &       &       &       &       &        &       \\
OCSVM        &    ++ &          ++ &      ++ &   ++ &  ++ &       ++ &   ++ &     &              &       &       &       &       &       &       &       &          &       &       &       &       &       &         &       &         &       &       &       &       &       &        &       \\
AE           &    ++ &          ++ &      ++ &   ++ &     &       ++ &    + &     &              &       &       &       &       &       &       &       &          &       &       &       &       &       &         &       &         &       &       &       &       &       &        &       \\
LUNAR        &    ++ &          ++ &      ++ &   ++ &     &       ++ &    + &     &              &       &       &       &       &       &       &       &          &       &       &       &       &       &         &       &         &       &       &       &       &       &        &       \\
beta-VAE     &    ++ &          ++ &       + &   ++ &     &       ++ &      &     &              &       &       &       &       &       &       &       &          &       &       &       &       &       &         &       &         &       &       &       &       &       &   -\{\}- &       \\
VAE          &    ++ &          ++ &      ++ &   ++ &     &       ++ &      &     &              &       &       &       &       &       &       &       &          &       &       &       &       &       &         &       &         &       &       &       &       &       &      - &       \\
ECOD         &    ++ &          ++ &      ++ &   ++ &     &       ++ &    + &     &              &       &       &       &       &       &       &       &          &       &       &       &       &       &         &       &         &       &       &       &       &       &        &       \\
PCA          &       &          ++ &         &      &     &          &      &     &              &       &       &       &       &       &       &       &          &       &       &       &       &       &         &       &         &  -\{\}- &       &       &  -\{\}- &  -\{\}- &   -\{\}- &  -\{\}- \\
SOD          &    ++ &          ++ &         &      &     &          &      &     &              &       &       &       &       &       &       &       &          &       &       &       &       &       &         &       &         &     - &       &       &       &  -\{\}- &   -\{\}- &  -\{\}- \\
LODA         &     + &          ++ &         &      &     &          &      &     &              &       &       &       &       &       &       &       &          &       &       &       &       &       &         &       &         &  -\{\}- &       &       &     - &  -\{\}- &   -\{\}- &  -\{\}- \\
LMDD         &    ++ &          ++ &         &      &     &          &      &     &              &       &       &       &       &       &       &       &          &       &       &       &       &       &         &       &         &     - &       &       &       &  -\{\}- &   -\{\}- &  -\{\}- \\
GMM          &    ++ &          ++ &      ++ &   ++ &     &       ++ &    + &     &              &       &       &       &       &       &       &       &          &       &       &       &       &       &         &       &         &       &       &       &       &       &        &       \\
ensemble-LOF &       &          ++ &         &      &     &          &      &     &              &       &       &       &       &       &       &       &          &       &       &       &       &       &         &     - &         &  -\{\}- &       &       &  -\{\}- &  -\{\}- &   -\{\}- &  -\{\}- \\
LOF          &       &             &         &      &     &          &      &     &              &       &       &       &       &       &       &       &          &       &       &       &       &  -\{\}- &         &  -\{\}- &    -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &   -\{\}- &  -\{\}- \\
ODIN         &       &             &         &      &     &          &      &     &              &     - &       &       &       &       &     - &       &          &     - &     - &  -\{\}- &  -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &   -\{\}- &  -\{\}- \\
DeepSVDD     &       &             &         &      &     &          &      &     &              &  -\{\}- &       &       &       &       &  -\{\}- &  -\{\}- &     -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &   -\{\}- &  -\{\}- \\
COF          &       &             &         &      &     &          &      &     &              &       &       &       &       &       &       &       &          &       &       &  -\{\}- &  -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &   -\{\}- &  -\{\}- \\
ALAD         &       &             &         &      &     &          &      &     &              &  -\{\}- &       &       &       &       &  -\{\}- &  -\{\}- &     -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &   -\{\}- &  -\{\}- \\
SO-GAAL      &       &             &         &      &     &          &      &     &              &  -\{\}- &       &       &       &       &  -\{\}- &  -\{\}- &        - &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &   -\{\}- &  -\{\}- \\
sb-DeepSVDD  &       &             &         &      &     &          &      &     &         -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &     -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &   -\{\}- &  -\{\}- \\
CBLOF        &       &             &         &      &     &          &      &     &              &  -\{\}- &  -\{\}- &     - &  -\{\}- &       &  -\{\}- &  -\{\}- &     -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &   -\{\}- &  -\{\}- \\
\bottomrule
\end{tabular}


==> Tables/nemenyi_summary_global.tex <==
\begin{tabular}{lllllllllllllllllllllllllllllllll}
\toprule
{} & CBLOF & COF & sb-DeepSVDD & ODIN & ALAD & LOF & DeepSVDD & SO-GAAL & ensemble-LOF &   GMM & SOD & LUNAR &  LODA &  LMDD &  ABOD &   VAE &   PCA &   KDE &   kNN &  HBOS & u-CBLOF & beta-VAE &   MCD &  ECOD & OCSVM &    AE & kth-NN &  INNE & gen2out & COPOD &    IF &   EIF \\
\midrule
EIF          &    ++ &  ++ &          ++ &   ++ &   ++ &  ++ &       ++ &      ++ &           ++ &    ++ &  ++ &    ++ &    ++ &     + &       &       &     + &       &       &       &         &          &       &       &       &       &        &       &         &       &       &       \\
IF           &    ++ &  ++ &          ++ &   ++ &   ++ &  ++ &       ++ &      ++ &           ++ &     + &  ++ &    ++ &     + &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &       &       &       \\
COPOD        &    ++ &  ++ &          ++ &   ++ &   ++ &  ++ &       ++ &      ++ &           ++ &     + &  ++ &    ++ &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &       &       &       \\
gen2out      &    ++ &  ++ &          ++ &   ++ &   ++ &  ++ &       ++ &      ++ &           ++ &       &  ++ &       &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &       &       &       \\
INNE         &    ++ &  ++ &          ++ &   ++ &   ++ &  ++ &       ++ &      ++ &           ++ &       &  ++ &       &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &       &       &       \\
kth-NN       &    ++ &  ++ &          ++ &   ++ &   ++ &  ++ &       ++ &      ++ &           ++ &       &  ++ &       &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &       &       &       \\
AE           &    ++ &  ++ &          ++ &   ++ &   ++ &  ++ &       ++ &      ++ &           ++ &       &     &       &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &       &       &       \\
OCSVM        &    ++ &  ++ &          ++ &   ++ &   ++ &  ++ &       ++ &      ++ &           ++ &       &  ++ &       &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &       &       &       \\
ECOD         &    ++ &  ++ &          ++ &   ++ &   ++ &  ++ &       ++ &      ++ &           ++ &       &  ++ &       &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &       &       &       \\
MCD          &    ++ &  ++ &          ++ &   ++ &   ++ &  ++ &       ++ &      ++ &           ++ &       &  ++ &       &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &       &       &       \\
beta-VAE     &    ++ &  ++ &          ++ &   ++ &   ++ &  ++ &       ++ &      ++ &            + &       &     &       &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &       &       &       \\
u-CBLOF      &    ++ &  ++ &          ++ &   ++ &   ++ &  ++ &       ++ &      ++ &            + &       &     &       &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &       &       &       \\
HBOS         &    ++ &  ++ &          ++ &   ++ &   ++ &  ++ &       ++ &      ++ &           ++ &       &  ++ &       &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &       &       &       \\
kNN          &    ++ &  ++ &          ++ &   ++ &   ++ &  ++ &       ++ &      ++ &           ++ &       &  ++ &       &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &       &       &       \\
KDE          &    ++ &  ++ &          ++ &   ++ &   ++ &  ++ &       ++ &      ++ &           ++ &       &  ++ &       &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &       &       &       \\
PCA          &    ++ &  ++ &          ++ &   ++ &   ++ &  ++ &       ++ &         &              &       &     &       &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &       &       &     - \\
VAE          &    ++ &  ++ &          ++ &   ++ &   ++ &  ++ &       ++ &       + &              &       &     &       &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &       &       &       \\
ABOD         &    ++ &  ++ &          ++ &   ++ &   ++ &  ++ &       ++ &      ++ &              &       &     &       &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &       &       &       \\
LMDD         &    ++ &  ++ &          ++ &   ++ &   ++ &  ++ &       ++ &         &              &       &     &       &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &       &       &     - \\
LODA         &    ++ &  ++ &          ++ &   ++ &      &     &        + &         &              &       &     &       &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &       &     - &  -\{\}- \\
LUNAR        &    ++ &  ++ &          ++ &   ++ &      &     &          &         &              &       &     &       &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &  -\{\}- &  -\{\}- &  -\{\}- \\
SOD          &       &     &             &      &      &     &          &         &              &       &     &       &       &       &       &       &       &  -\{\}- &  -\{\}- &  -\{\}- &         &          &  -\{\}- &  -\{\}- &  -\{\}- &       &   -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- \\
GMM          &    ++ &  ++ &          ++ &   ++ &      &     &          &         &              &       &     &       &       &       &       &       &       &       &       &       &         &          &       &       &       &       &        &       &         &     - &     - &  -\{\}- \\
ensemble-LOF &       &     &             &      &      &     &          &         &              &       &     &       &       &       &       &       &       &  -\{\}- &  -\{\}- &  -\{\}- &       - &        - &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &   -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- \\
SO-GAAL      &       &     &             &      &      &     &          &         &              &       &     &       &       &       &  -\{\}- &     - &       &  -\{\}- &  -\{\}- &  -\{\}- &    -\{\}- &     -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &   -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- \\
DeepSVDD     &       &     &             &      &      &     &          &         &              &       &     &       &     - &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &    -\{\}- &     -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &   -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- \\
LOF          &       &     &             &      &      &     &          &         &              &       &     &       &       &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &    -\{\}- &     -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &   -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- \\
ALAD         &       &     &             &      &      &     &          &         &              &       &     &       &       &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &    -\{\}- &     -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &   -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- \\
ODIN         &       &     &             &      &      &     &          &         &              &  -\{\}- &     &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &    -\{\}- &     -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &   -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- \\
sb-DeepSVDD  &       &     &             &      &      &     &          &         &              &  -\{\}- &     &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &    -\{\}- &     -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &   -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- \\
COF          &       &     &             &      &      &     &          &         &              &  -\{\}- &     &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &    -\{\}- &     -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &   -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- \\
CBLOF        &       &     &             &      &      &     &          &         &              &  -\{\}- &     &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &    -\{\}- &     -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &   -\{\}- &  -\{\}- &    -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- \\
\bottomrule
\end{tabular}


==> Tables/nemenyi_summary_local.tex <==
\begin{tabular}{lllllllllllllllllllllllllllllllll}
\toprule
{} & SO-GAAL & PCA & ECOD & beta-VAE & ALAD & LMDD & COPOD &  AE & LODA & OCSVM & sb-DeepSVDD & DeepSVDD & VAE & HBOS & CBLOF & gen2out & IF & EIF & INNE & u-CBLOF & ODIN & LUNAR &   MCD &   KDE &   GMM &   SOD &   COF &   LOF & ensemble-LOF & kth-NN &  ABOD &   kNN \\
\midrule
kNN          &      ++ &  ++ &   ++ &       ++ &   ++ &   ++ &    ++ &  ++ &   ++ &    ++ &          ++ &       ++ &  ++ &   ++ &    ++ &      ++ &    &     &      &         &      &       &       &       &       &       &       &       &              &        &       &       \\
ABOD         &      ++ &  ++ &   ++ &       ++ &   ++ &   ++ &    ++ &  ++ &   ++ &    ++ &          ++ &       ++ &  ++ &   ++ &    ++ &      ++ &    &     &      &         &      &       &       &       &       &       &       &       &              &        &       &       \\
kth-NN       &      ++ &  ++ &   ++ &       ++ &   ++ &   ++ &    ++ &  ++ &   ++ &    ++ &          ++ &        + &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &       &              &        &       &       \\
ensemble-LOF &      ++ &  ++ &   ++ &       ++ &   ++ &   ++ &    ++ &  ++ &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &       &              &        &       &       \\
LOF          &      ++ &  ++ &   ++ &       ++ &   ++ &   ++ &    ++ &  ++ &    + &     + &           + &          &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &       &              &        &       &       \\
COF          &      ++ &  ++ &   ++ &       ++ &   ++ &   ++ &    ++ &  ++ &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &       &              &        &       &       \\
SOD          &      ++ &  ++ &   ++ &       ++ &   ++ &   ++ &    ++ &  ++ &      &     + &           + &          &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &       &              &        &       &       \\
GMM          &      ++ &  ++ &   ++ &       ++ &      &   ++ &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &       &              &        &       &       \\
KDE          &      ++ &  ++ &   ++ &       ++ &   ++ &   ++ &    ++ &  ++ &      &       &           + &          &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &       &              &        &       &       \\
MCD          &         &  ++ &    + &        + &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &       &              &        &       &       \\
LUNAR        &      ++ &  ++ &   ++ &       ++ &      &   ++ &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &       &              &        &       &       \\
ODIN         &         &   + &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &       &              &        &       &       \\
u-CBLOF      &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &       &              &        &       &       \\
INNE         &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &       &              &        &       &       \\
EIF          &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &       &              &        &       &       \\
IF           &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &       &              &        &       &       \\
gen2out      &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &       &              &        &  -\{\}- &  -\{\}- \\
CBLOF        &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &       &              &        &  -\{\}- &  -\{\}- \\
HBOS         &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &       &              &        &  -\{\}- &  -\{\}- \\
VAE          &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &       &              &        &  -\{\}- &  -\{\}- \\
DeepSVDD     &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &       &              &      - &  -\{\}- &  -\{\}- \\
sb-DeepSVDD  &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &     - &       &     - &       &     - &              &   -\{\}- &  -\{\}- &  -\{\}- \\
OCSVM        &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &       &       &     - &       &     - &              &   -\{\}- &  -\{\}- &  -\{\}- \\
LODA         &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &       &       &       &       &     - &              &   -\{\}- &  -\{\}- &  -\{\}- \\
AE           &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &  -\{\}- &       &  -\{\}- &  -\{\}- &  -\{\}- &         -\{\}- &   -\{\}- &  -\{\}- &  -\{\}- \\
COPOD        &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &  -\{\}- &       &  -\{\}- &  -\{\}- &  -\{\}- &         -\{\}- &   -\{\}- &  -\{\}- &  -\{\}- \\
LMDD         &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &  -\{\}- &       &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &         -\{\}- &   -\{\}- &  -\{\}- &  -\{\}- \\
ALAD         &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &       &       &  -\{\}- &       &  -\{\}- &  -\{\}- &  -\{\}- &         -\{\}- &   -\{\}- &  -\{\}- &  -\{\}- \\
beta-VAE     &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &  -\{\}- &     - &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &         -\{\}- &   -\{\}- &  -\{\}- &  -\{\}- \\
ECOD         &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &  -\{\}- &     - &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &         -\{\}- &   -\{\}- &  -\{\}- &  -\{\}- \\
PCA          &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &    - &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &         -\{\}- &   -\{\}- &  -\{\}- &  -\{\}- \\
SO-GAAL      &         &     &      &          &      &      &       &     &      &       &             &          &     &      &       &         &    &     &      &         &      &  -\{\}- &       &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &  -\{\}- &         -\{\}- &   -\{\}- &  -\{\}- &  -\{\}- \\
\bottomrule
\end{tabular}


==> Tables/significance_results_all_datasets.tex <==
\begin{tabular}{lrrrl}
\toprule
{} &  Mean Performance &  Performance std &  Performance Range &                                        Outperforms \\
\midrule
EIF          &            0.7725 &           0.1656 &             0.6248 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
kth-NN       &            0.7693 &           0.1575 &             0.5903 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
kNN          &            0.7655 &           0.1567 &             0.5906 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
IF           &            0.7636 &           0.1654 &             0.6263 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
MCD          &            0.7564 &           0.1765 &             0.6333 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
INNE         &            0.7494 &           0.1692 &             0.6820 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
KDE          &            0.7483 &           0.1959 &             0.9178 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
gen2out      &            0.7477 &           0.1737 &             0.5866 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
ABOD         &            0.7475 &           0.1760 &             0.8131 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
u-CBLOF      &            0.7412 &           0.1671 &             0.6135 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, ODIN, COF, ... \\
COPOD        &            0.7378 &           0.1808 &             0.6501 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
HBOS         &            0.7253 &           0.1767 &             0.6523 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, ODIN, COF, ... \\
OCSVM        &            0.7229 &           0.1855 &             0.6210 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, ODIN, COF, ... \\
AE           &            0.7200 &           0.1900 &             0.6668 &        CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, DeepSVDD \\
LUNAR        &            0.7112 &           0.1491 &             0.5698 &        CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, DeepSVDD \\
beta-VAE     &            0.7105 &           0.1888 &             0.6690 &                 CBLOF, sb-DeepSVDD, ALAD, DeepSVDD \\
VAE          &            0.7100 &           0.1600 &             0.6673 &        CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, DeepSVDD \\
ECOD         &            0.7095 &           0.1877 &             0.6291 &        CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, DeepSVDD \\
PCA          &            0.6921 &           0.2051 &             0.6928 &                                        sb-DeepSVDD \\
SOD          &            0.6869 &           0.1466 &             0.5718 &                                 CBLOF, sb-DeepSVDD \\
LODA         &            0.6848 &           0.1854 &             0.8165 &                                        sb-DeepSVDD \\
LMDD         &            0.6838 &           0.1900 &             0.6392 &                                 CBLOF, sb-DeepSVDD \\
GMM          &            0.6825 &           0.1904 &             0.8575 &        CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, DeepSVDD \\
ensemble-LOF &            0.6606 &           0.1512 &             0.6005 &                                        sb-DeepSVDD \\
LOF          &            0.6298 &           0.1320 &             0.5805 &                                                    \\
ODIN         &            0.5955 &           0.1140 &             0.4435 &                                                    \\
DeepSVDD     &            0.5932 &           0.1194 &             0.5216 &                                                    \\
COF          &            0.5923 &           0.1317 &             0.5510 &                                                    \\
ALAD         &            0.5694 &           0.1168 &             0.5499 &                                                    \\
SO-GAAL      &            0.5636 &           0.2247 &             0.8796 &                                                    \\
sb-DeepSVDD  &            0.5532 &           0.1069 &             0.5819 &                                                    \\
CBLOF        &            0.5192 &           0.1538 &             0.7767 &                                                    \\
\bottomrule
\end{tabular}


==> Tables/significance_results_global.tex <==
\begin{tabular}{lrrrl}
\toprule
{} &  Mean Performance &  Performance std &  Performance Range &                                        Outperforms \\
\midrule
EIF          &            0.8238 &           0.1348 &             0.5279 &  GMM, CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, O... \\
IF           &            0.8143 &           0.1365 &             0.5309 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
COPOD        &            0.8092 &           0.1324 &             0.5037 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
gen2out      &            0.8005 &           0.1544 &             0.5410 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
INNE         &            0.7899 &           0.1491 &             0.5287 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
kth-NN       &            0.7845 &           0.1556 &             0.5903 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
AE           &            0.7822 &           0.1541 &             0.5308 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
OCSVM        &            0.7811 &           0.1607 &             0.5324 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
ECOD         &            0.7801 &           0.1468 &             0.5079 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
MCD          &            0.7790 &           0.1713 &             0.6018 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
beta-VAE     &            0.7789 &           0.1500 &             0.5305 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
u-CBLOF      &            0.7756 &           0.1550 &             0.5302 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
HBOS         &            0.7740 &           0.1650 &             0.6523 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
kNN          &            0.7739 &           0.1559 &             0.5906 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
KDE          &            0.7663 &           0.2012 &             0.9178 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
PCA          &            0.7626 &           0.1686 &             0.5306 &  CBLOF, sb-DeepSVDD, ALAD, LOF, ODIN, COF, Deep... \\
VAE          &            0.7576 &           0.1371 &             0.5307 &  CBLOF, sb-DeepSVDD, ALAD, LOF, ODIN, COF, Deep... \\
ABOD         &            0.7524 &           0.1832 &             0.8131 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, LOF, ODIN, ... \\
LMDD         &            0.7382 &           0.1796 &             0.5841 &  CBLOF, sb-DeepSVDD, ALAD, LOF, ODIN, COF, Deep... \\
LODA         &            0.7338 &           0.1549 &             0.5052 &                      CBLOF, sb-DeepSVDD, ODIN, COF \\
LUNAR        &            0.7223 &           0.1438 &             0.5698 &                      CBLOF, sb-DeepSVDD, ODIN, COF \\
SOD          &            0.6791 &           0.1427 &             0.5718 &                                                    \\
GMM          &            0.6767 &           0.1962 &             0.8575 &                      CBLOF, sb-DeepSVDD, ODIN, COF \\
ensemble-LOF &            0.6433 &           0.1382 &             0.5581 &                                                    \\
SO-GAAL      &            0.6093 &           0.2063 &             0.7769 &                                                    \\
DeepSVDD     &            0.6050 &           0.1224 &             0.5216 &                                                    \\
LOF          &            0.6027 &           0.1031 &             0.5205 &                                                    \\
ALAD         &            0.5885 &           0.1167 &             0.5499 &                                                    \\
ODIN         &            0.5707 &           0.0809 &             0.3536 &                                                    \\
sb-DeepSVDD  &            0.5557 &           0.1155 &             0.5819 &                                                    \\
COF          &            0.5533 &           0.0891 &             0.4674 &                                                    \\
CBLOF        &            0.5004 &           0.1611 &             0.7767 &                                                    \\
\bottomrule
\end{tabular}


==> Tables/significance_results_local.tex <==
\begin{tabular}{lrrrl}
\toprule
{} &  Mean Performance &  Performance std &  Performance Range &                                        Outperforms \\
\midrule
kNN          &            0.7397 &           0.1631 &             0.4916 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, AE, COPOD, ... \\
ABOD         &            0.7325 &           0.1579 &             0.4640 &  CBLOF, SO-GAAL, sb-DeepSVDD, ALAD, AE, COPOD, ... \\
kth-NN       &            0.7222 &           0.1604 &             0.4957 &  SO-GAAL, sb-DeepSVDD, ALAD, AE, COPOD, beta-VA... \\
ensemble-LOF &            0.7141 &           0.1821 &             0.5069 &  SO-GAAL, ALAD, AE, COPOD, beta-VAE, PCA, ECOD,... \\
LOF          &            0.7134 &           0.1763 &             0.4865 &  SO-GAAL, ALAD, AE, COPOD, beta-VAE, PCA, ECOD,... \\
COF          &            0.7125 &           0.1698 &             0.4454 &  SO-GAAL, ALAD, AE, COPOD, beta-VAE, PCA, ECOD,... \\
SOD          &            0.7107 &           0.1621 &             0.4905 &  SO-GAAL, ALAD, AE, COPOD, beta-VAE, PCA, ECOD,... \\
GMM          &            0.7006 &           0.1782 &             0.5902 &                 SO-GAAL, beta-VAE, PCA, ECOD, LMDD \\
KDE          &            0.6930 &           0.1748 &             0.5474 &  SO-GAAL, ALAD, AE, COPOD, beta-VAE, PCA, ECOD,... \\
MCD          &            0.6865 &           0.1812 &             0.5830 &                                                PCA \\
LUNAR        &            0.6772 &           0.1664 &             0.4515 &                 SO-GAAL, beta-VAE, PCA, ECOD, LMDD \\
ODIN         &            0.6720 &           0.1639 &             0.4435 &                                                    \\
u-CBLOF      &            0.6353 &           0.1645 &             0.4829 &                                                    \\
INNE         &            0.6243 &           0.1720 &             0.5808 &                                                    \\
EIF          &            0.6143 &           0.1548 &             0.5066 &                                                    \\
IF           &            0.6074 &           0.1523 &             0.4858 &                                                    \\
gen2out      &            0.5848 &           0.1237 &             0.3463 &                                                    \\
CBLOF        &            0.5772 &           0.1158 &             0.3984 &                                                    \\
HBOS         &            0.5753 &           0.1213 &             0.3969 &                                                    \\
VAE          &            0.5633 &           0.1383 &             0.5033 &                                                    \\
DeepSVDD     &            0.5571 &           0.1065 &             0.3289 &                                                    \\
sb-DeepSVDD  &            0.5456 &           0.0784 &             0.2994 &                                                    \\
OCSVM        &            0.5434 &           0.1382 &             0.4628 &                                                    \\
LODA         &            0.5340 &           0.1962 &             0.7639 &                                                    \\
AE           &            0.5281 &           0.1631 &             0.4853 &                                                    \\
COPOD        &            0.5177 &           0.1235 &             0.4574 &                                                    \\
LMDD         &            0.5162 &           0.1072 &             0.3778 &                                                    \\
ALAD         &            0.5108 &           0.1000 &             0.3842 &                                                    \\
beta-VAE     &            0.4994 &           0.1325 &             0.4662 &                                                    \\
ECOD         &            0.4918 &           0.1214 &             0.4017 &                                                    \\
PCA          &            0.4747 &           0.1489 &             0.4912 &                                                    \\
SO-GAAL      &            0.4228 &           0.2289 &             0.7616 &                                                    \\
\bottomrule
\end{tabular}

